A Heterogeneous RISC-V based SoC for Secure Nano-UAV Navigation

The rapid advancement of energy-efficient parallel ultra-low-power (ULP) ucontrollers units (MCUs) is enabling the development of autonomous nano-sized unmanned aerial vehicles (nano-UAVs). These sub-10cm drones represent the next generation of unobtrusive robotic helpers and ubiquitous smart sensors. However, nano-UAVs face significant power and payload constraints while requiring advanced computing capabilities akin to standard drones, including real-time Machine Learning (ML) performance and the safe co-existence of general-purpose and real-time OSs. Although some advanced parallel ULP MCUs offer the necessary ML computing capabilities within the prescribed power limits, they rely on small main memories (<1MB) and ucontroller-class CPUs with no virtualization or security features, and hence only support simple bare-metal runtimes. In this work, we present Shaheen, a 9mm2 200mW SoC implemented in 22nm FDX technology. Differently from state-of-the-art MCUs, Shaheen integrates a Linux-capable RV64 core, compliant with the v1.0 ratified Hypervisor extension and equipped with timing channel protection, along with a low-cost and low-power memory controller exposing up to 512MB of off-chip low-cost low-power HyperRAM directly to the CPU. At the same time, it integrates a fully programmable energy- and area-efficient multi-core cluster of RV32 cores optimized for general-purpose DSP as well as reduced- and mixed-precision ML. To the best of the authors' knowledge, it is the first silicon prototype of a ULP SoC coupling the RV64 and RV32 cores in a heterogeneous host+accelerator architecture fully based on the RISC-V ISA. We demonstrate the capabilities of the proposed SoC on a wide range of benchmarks relevant to nano-UAV applications. The cluster can deliver up to 90GOp/s and up to 1.8TOp/s/W on 2-bit integer kernels and up to 7.9GFLOp/s and up to 150GFLOp/s/W on 16-bit FP kernels.

==> authors/Authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/luca_v.jpg}}]{Luca Valente} received the MSc degree in electronic engineering from the Politecnico of Turin in 2020. He is currently a PhD student at the University of Bologna within the Department of Electrical, Electronic and Information Technologies Engineering (DEI). His main research interests are hardware-software co-design of multi-processors heterogenous systems on chip, parallel programming and FPGA prototyping.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/anadalini.jpg}}]{Alessandro Nadalini} received the B.Sc. and M.Sc. degrees in electronic engineering from the University of Bologna, Bologna, Italy, in 2018 and 2021, respectively. He currently holds a research grant from the University of Bologna. His research regards lightweight extensions to the RISC-V ISA to boost the efficiency of heavily quantized neural networks inference on microcontroller-class cores. He received the Mukherjee Best Paper Award of the 2023 IEEE Computer Society Annual Symposium on VLSI.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/asif.jpg}}]{Asif Hussain Chiralil Veeran} is a researcher in the field of Electrical Engineering and Computer Science (EECS) at Khalifa University. He obtained his Master of Science (M.S.) in VLSI Design from Anna University, India, and a Bachelor of Science (B.S.) in Electronics and Communication Engineering from the University of Calicut. His research interests encompass VLSI, developing efficient and effective methodologies and designing and optimising the layout of ICs, ensuring their functionality, performance, and manufacturability.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/smatt.jpg}}]{Mattia Sinigaglia} received his Master’s Degree in Electronic Engineering from the University of Bologna. He is currently pursuing a Ph. D. in Digital Systems Design in the group of Professor Luca Benini at the Department of Electrical and Information Engineering (DEI) of the University of Bologna.  His research interest is semiconductor engineering for ultra-low-power devices, mainly targeting hardware-software co-design of heterogeneous System on Chip.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/ninolomata.jpg}}]{Bruno Sà} is a Ph.D. student at the  Embedded  Systems  Research Group, University of Minho, Portugal. Bruno holds a Master in Electronics and Computer Engineering with specialization in Embedded Systems and Automation,Control and Robotics. Bruno's areas of interest include operating systems and virtualization for embedded critical systems, computer architectures, hardware-software co-design. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/Nils.png}}]{Nils Wistoff} received the BSc and MSc degrees from RWTH Aachen University in 2017 and 2020, respectively. He is currently working toward the PhD degree with the Integrated Systems Laboratory of ETH Zurich. His research interests include processor and system-on-chip design and secure computer architecture.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/yvan.jpg}}]{Yvan Tortorella} received his Master’s Degree in Electronic Engineering in October 2021 from the University of Bologna. He is currently pursuing a Ph. D. in Digital Systems Design in the group of Professor Luca Benini at the Department of Electrical and Information Engineering (DEI) of the University of Bologna. His research interests include the design of PULP (Parallel Ultra-Low Power)-based hardware accelerators for ultra-low power Machine Learning and the design of RISC-V-based computer architectures for satellite applications. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/sbenatti.png}}]{Simone Benatti} received the Ph.D. degree in electrical engineering and computer science from the University of Bologna, Bologna, Italy, in 2016. He has collaborated with several international research institutes and companies. Previously, he worked for 8 years as an Electronic Designer and R\&D Engineer of electromedical devices. He has authored or coauthored more than 50 papers in international peer-reviewed conferences and journals. His research interests focus on energy efﬁcient embedded wearable systems, signal processing, sensor fusion, and actuation systems. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/rafail.png}}]{Rafail Psiakis} holds a Ph.D. degree from University of Rennes, France, obtained in 2018, and a M.S. \& Bachelor joint diploma from the Department of Electrical and Computer Engineering at University of Patras, Greece, obtained in 2015. Currently he is a Lead Silicon Security Researcher at Technology Innovation Institute, Abu Dhabi, UAE. Previously, he worked 5 years as an Embedded R\&D Security Engineer and Research Assistant. His research interests include embedded systems, security, confidential computing, computer architecture, RISC-V, fault tolerance.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/ari.jpg}}]{Ari Kulmala} received his Ph.D. degree in 2009 from the Tampere University of Technology (TUT). Currently he is leading the SoC Development at Technology Innovation Institute (TII) Secure Systems Research Center of Abu Dhabi and holds the position of Professor of Practice at Tampere University of Technology. His experience on System-on-Chip design ranges from small power mobile devices to large scale processing infrastructure devices and datacenter applications. %After working 2003-2008 in Tampere University of Technology, in 2009, he joined Wireless Modem unit of Devices R\&D in Nokia as technical digital ASIC project manager. Then he worked with Renesas Electronics (Renesas Mobile) from 2010-2013 with wireless SoC development. In 2013 he joined Nokia Networks and headed several organizations with experience from radio and baseband to datacenter hardware. In 2020 he joined part-time Tampere University and in 2021 Nordic Semiconductor for heading a Digital IC site establishment for wireless IoT SoC development.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/baker.jpg}}]{Baker Mohammad} holds a PhD in Electrical and Computer Engineering (ECE) from the University of Texas at Austin and an M.S. in ECE from Arizona State University, Tempe a B.S. degree in ECE from the University of New Mexico, Albuquerque. He is a distinguished lecturer of IEEE CAS. Dr Mohammad is currently a professor of Electrical Engineering and Computer Science (EECS) at Khalifa University and is the director of the SOCL.  % Before joining Khalifa University, Dr. Baker worked for 16 years in the US industry (Qualcomm \& Intel). % designing low-power and high-performance processors. %Baker’s research interests include VLSI, power-efficient computing, high-yield embedded memory, and emerging technologies such as Memristor, STTRAM, In-Memory-Computing, Hardware accelerators and power management. 
Dr. Baker has authored or co-authored over 200 referred journals and conference proceedings, more than three books, and over 20 U.S. patents.  
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/SandroPinto.jpg}}]{Sandro Pinto} is an Associate Research Professor at the University of Minho, Portugal. He holds a Ph.D. in Electronics and Computer Engineering. Dr. Sandro has a deep academic background and several years of industry collaboration focusing on operating systems, virtualization, and security for embedded, CPS, and IoT systems. He has published 80+ peer-reviewed papers and is a skilled presenter with speaking experience in several academic and industrial conferences. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/dpalossi.png}}]{Daniele Palossi} received his Ph.D. from the ETH Z\"urich in 2019. He is currently a Senior Researcher at the Dalle Molle Institute for Artificial Intelligence (IDSIA), USI-SUPSI, Lugano, Switzerland, and at the Integrated Systems Laboratory (IIS), ETH Zürich, Zürich, Switzerland. His research focuses on energy-efficient embedded platforms, algorithms for autonomous navigation, and miniaturized cyber-physical systems. His work has resulted in 30+ publications in international peer-reviewed conferences and journals. Dr. Palossi was a recipient of the Swiss National Science Foundation (SNSF) Spark Grant, the 2nd prize at the Design Contest held at the ACM/IEEE ISLPED'19, and led the winning team of the first ``Nanocopter AI Challenge`` at the IMAV'22 International Conference.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/luca_benini.jpg}}]{Luca Benini} holds the chair of digital Circuits and systems at ETHZ and is Full Professor at the Universit\`{a} di Bologna. He received a PhD from Stanford University. Dr. Benini’s research interests are in energy-efficient parallel computing systems, smart sensing micro-systems and machine learning hardware. He has published more than 1000 peer-reviewed papers and five books. He is a Fellow of the ACM and a member of the Academia Europaea.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/DAVIDE_ROSSI.png}}]{Davide Rossi} received the Ph.D. degree from the University of Bologna, Bologna, Italy, in 2012. He has been a Post-Doctoral Researcher with the Department of Electrical, Electronic and Information Engineering “Guglielmo Marconi,” University of Bologna, since 2015, where he is currently an Assistant Professor. His research interests focus on energy-efficient digital architectures. In this field, he has published more than 100 papers in international peer-reviewed conferences and journals. He is recipient of Donald O. Pederson Best Paper Award 2018, 2020 IEEE TCAS Darlington Best Paper Award, 2020 IEEE TVLSI Prize Paper Award.
\end{IEEEbiography}

\vfill
